Dark Z at the International Linear Collider

A dark Z is a massive Abelian gauge boson which is coupled to the Standard Model through both kinetic and mass mixing with the electroweak sector. We study the phenomenology of the dark Z at an energy-frontier electron-positron collider, such as the proposed International Linear Collider (ILC). We show that precision electroweak constraints and the current bounds from the hadron colliders allow a dark Z that is kinematically accessible at the ILC with 250 GeV or 500 GeV center-of-mass energy. Further, the reach of the ILC searches for a dark Z significantly exceeds the expected reach of the high luminosity LHC. If a signal consistent with a dark Z is discovered, it would motivate a dedicated run of the ILC at the center-of-mass energy matching the dark Z mass. We demonstrate that a short one month run at design luminosity could measure the dark Z chiral couplings to fermions with percent precision. This measurement can be used to discriminate between competing theoretical models of the resonance: for example, the dark Z can be distinguished from a dark photon with purely kinetic mixing.

==> FlipAdditionalHeader.tex <==
%!TEX root = paper.tex
%% Update the above with the appropriate root

%% Place additional project-specific macros, package calls here
%% These are called before FlipPreambleEnd.tex so that,
%% for example, they are called before hyperref

%% Example: replace YourName with your name
\newcommand{\YourName}[1]{{	
	\color{blue!50!black}\footnotesize
	[\textbf{\textsf{YourName}}: \textsf{#1}]}}
